Combine User's Manual

{\sc Combine} is an add-on to {\sc SigSpec} and {\sc Cinderella}. A {\sc SigSpec} result file or a file generated by {\sc Cinderella} contains the significant sinusoidal signal components in a time series. In this file, {\sc Combine} checks one frequency after the other for being a linear combination of previously examined frequencies. If this attempt fails, the corresponding frequency is considered ``genuine''. Only genuine frequencies are used to form linear combinations subsequently. A purely heuristic model is employed to assign a reliability to each linear combination and to justify whether to consider a frequency genuine or a linear combination.

==> CoAst_layo.tex <==
\pagestyle{fancyplain}
\addtolength{\headwidth}{\marginparsep}
\addtolength{\headwidth}{\marginparwidth}
\addtolength{\headwidth}{\marginparwidth}
\renewcommand{\chaptermark}[1]{\markboth{#1}{}}
\renewcommand{\sectionmark}[1]{\markright{#1}}
\lhead[\fancyplain{}{\sffamily\thepage}]{\fancyplain{}{\sffamily}}
\rhead[\fancyplain{}{\sffamily\leftmark}]{\fancyplain{}{\sffamily\thepage}}
%\rfoot[]{\fancyplain{}{\sffamily\small Communications in Asteroseismology, No. 131, July 2001}}
%\lfoot[\fancyplain{}{\sffamily\small Communications in Asteroseismology, No. 131, July 2001}]{}
\cfoot{}
%\paperheight=230mm
%\paperwidth=150mm
\hoffset=-1cm
\voffset=1mm
\topmargin=-12mm
\headheight=5mm
\headwidth=115mm
\headsep=7mm
\oddsidemargin=1mm
\evensidemargin=1mm
\marginparwidth=0cm
\marginparsep=0cm
\renewcommand{\headrulewidth}{0pt}
\textwidth=115mm
\textheight=165mm
\footskip=10mm
\newcommand{\apj}{ApJ}
\newcommand{\aj}{AJ}  %************Stimmts?
\newcommand{\aap}{A\&A}  %*************Stimmts?
\newcommand{\mnras}{MNRAS}
\newcommand{\tspace}{\hspace{1.2em}}
\newcommand{\feh}{$[Fe/H]$}
\newcommand{\by}{\ensuremath{(b-y)}}       % b-y index
\newcommand{\nr}{\multicolumn{-1}{c}{\ensuremath{\lesssim 25}}}
\newcommand{\dss}{$\delta$~Scuti stars}                     % Style for Delta Scuti Stars (plur.)
\newcommand{\ds}{$\delta$~Scuti star}
\newcommand{\ngc}[1]{NGC~{#1}}                              % Style for NGCxxxx
\newcommand{\templogg}{\texttt{templogg}}                   % Style for "templogg" program name
\newcommand{\teff}{\ensuremath{T_{eff}}}             % T_eff
\newcommand{\logg}{\ensuremath{\log g}}                     % log g
\newcommand{\vsini}{\ensuremath{v\sin i}}                   % v sin 
\newcommand{\halpha}{H$\alpha$}  % H alpha
\def\kms {km~s$^{-1}$}
\def\kmss {km~s$^{-1}$~}
\def\cd {d$^{-1}$}

\newcommand{\kopf}{\small\itshape Comm. in Asteroseismology\\ 2008, in preparation}
\newcommand{\Authors}[1]{\begin{center}\normalsize\bf\sf #1 \end{center}}
\newcommand{\authors}[1]{\begin{center}\normalsize\bf\sf #1 \end{center}}
\newcommand{\Author}[1]{\begin{center}\normalsize\bf\sf #1 \end{center}}
\renewcommand{\author}[1]{\begin{center}\normalsize\bf\sf #1 \end{center}}
\newcommand{\Address}[1]{\begin{center}\small\sf #1 \end{center}}
\newcommand{\address}[1]{\begin{center}\small\sf #1 \end{center}}
\renewenvironment{abstract}{\section*{Abstract}\normalsize\sf}{}
\newcommand{\References}[1]{\begin{flushleft}{\large References\\}\vspace*{2mm}\small #1 \end{flushleft}}
%\newcommand{\references}[1]{\begin{flushleft}{\large References\\}\vspace*{2mm}\small #1 \end{flushleft}}

\newcommand{\chapterDSSN}[2]{\chapter[\sf\normalsize #1\\ \footnotesize \hspace*{5mm}by #2 \sf\normalsize][]{#1\\}\rhead[\fancyplain{}{\sf\footnotesize \center{#1}}]{\fancyplain{}{\sffamily\thepage}}\lhead[\fancyplain{\kopf}{\sffamily\thepage}]{\fancyplain{\kopf}{\sf\footnotesize \center{#2}}}}

\newcommand{\headDSSN}[2]{\rhead[\fancyplain{}{\sf\footnotesize \center{#1}}]{\fancyplain{}{\sffamily\thepage}}\lhead[\fancyplain{\kopf}{\sffamily\thepage}]{\fancyplain{\kopf}{\sf\footnotesize \center{#2}}}}

\newcommand{\chapterdssn}[2]{\chapter[\sf\normalsize #1\\ \footnotesize \hspace*{5mm}by #2 \sf\normalsize][]{#1\\}\rhead[\fancyplain{}{\sf\footnotesize \center{#1}}]{\fancyplain{}{\sffamily\thepage}}\lhead[\fancyplain{\kopf}{\sffamily\thepage}]{\fancyplain{\kopf}{\sf\footnotesize \center{#2}}}}

\newcommand{\headdssn}[2]{\rhead[\fancyplain{}{\sf\footnotesize \center{#1}}]{\fancyplain{}{\sffamily\thepage}}\lhead[\fancyplain{\kopf}{\sffamily\thepage}]{\fancyplain{\kopf}{\sf\footnotesize \center{#2}}}}

\newcommand{\figureDSSN}[5]{\begin{figure}[#4]
\centering
\includegraphics*[#5]{#1}
\caption{#2}
\label{#3}
\end{figure}}
\newcommand{\figuredssn}[5]{\begin{figure}[#4]
\centering
\includegraphics*[#5]{#1}
\caption{#2}
\label{#3}
\end{figure}}
\newcommand {\strich} {\begin{center} \vspace{0.5cm} \rule{1.5cm}{0.3mm} \end{center}}
\renewcommand{\chaptername}{}
\newcommand{\acknowledgments}[1]{\vspace*{5mm}\noindent\begin{bf}Acknowledgments. \end{bf} #1}
\newcommand{\acknowledgements}[1]{\vspace*{5mm}\noindent\begin{bf}Acknowledgments. \end{bf} #1}
\newcommand{\Acknowledgments}[1]{\vspace*{5mm}\noindent\begin{bf}Acknowledgments. \end{bf} #1}
\newcommand{\Acknowledgements}[1]{\vspace*{5mm}\noindent\begin{bf}Acknowledgments. \end{bf} #1}


==> caput_coast.tex <==


%%Version 1: this style won't cause trouble while compiling. it gives the name of the section and the stiff sheet
%\newpage
%\lhead[\fancyplain]{\fancyplain{}{}} \rhead[\fancyplain]{\fancyplain{}{}}
%\sectionheading{News \& Announcements}
%\newpage


%%Version 2: this will only give the stiff sheet. the section heading in the TOC has to be inserted with the command given below. Yet this will cause trouble when compiling the masterfile.
%\addtocontents{toc}{\vspace{1cm} \large\textbf{Recent Communications} \vspace{0cm} \normalsize} 

\newpage 

\thispagestyle{empty}
\vspace*{30mm}
\begin{center}
\huge CoAst  \\ Announcements \\
\end{center}



==> caput_editorialcomment.tex <==


%%Version 1: this style won't cause trouble while compiling. it gives the name of the section and the stiff sheet
%\newpage
%\lhead[\fancyplain]{\fancyplain{}{}} \rhead[\fancyplain]{\fancyplain{}{}}
%\sectionheading{News \& Announcements}
%\newpage


%%Version 2: this will only give the stiff sheet. the section heading in the TOC has to be inserted with the command given below. Yet this will cause trouble when compiling the masterfile.
%\addtocontents{toc}{\vspace{1cm} \large\textbf{Recent Communications} \vspace{0cm} \normalsize} 

\newpage 

\thispagestyle{empty}
\vspace*{30mm}



\section*{Editorial statement for the following paper (entitled \\ {\it MOST found evidence for solar-type oscillations in the K2 giant star HD\,20884)} }
{\it \small The main message of the following paper is to report the detection of nonradial pulsation in a K giant. This is an important and controversial topic.

A key issue for this investigation is the reliability of the extracted frequencies. Your editor has spent his life with Fourier amplitude spectra of high-precision ground-based photometry. From that experience, Figure 3 of the paper
represents the natural result of instrumental instabilities and atmospheric transparency changes and does not deserve a second look. However, these are satellite observations without the typical ground-based difficulties -- but there may be different problems.

The statistical analyses can only help us in a limited way. It does not matter much whether one applies my favorite criterion of amplitude signal/noise ratio < 4, the SigSpec values, or another method. All these statistical analyses rely on assumptions of the nature of noise present in the data. Again, in ground-based photometry, we have found that the statistics are not reliable for low-frequency peaks. The obvious method to verify that certain peaks are not noise is to look at a comparison sample: the authors provide the results for another star with a simpler light curve. In my opinion, the issue is not yet solved.\normalsize}




==> caput_empty.tex <==


%%Version 1: this style won't cause trouble while compiling. it gives the name of the section and the stiff sheet
%\newpage
%\lhead[\fancyplain]{\fancyplain{}{}} \rhead[\fancyplain]{\fancyplain{}{}}
%\sectionheading{News \& Announcements}
%\newpage


%%Version 2: this will only give the stiff sheet. the section heading in the TOC has to be inserted with the command given below. Yet this will cause trouble when compiling the masterfile.
%\addtocontents{toc}{\vspace{1cm} \large\textbf{Recent Communications} \vspace{0cm} \normalsize} 

\newpage 

\thispagestyle{empty}
\vspace*{30mm}
\begin{center}
%here would come some text

\end{center}



==> caput_helas.tex <==


%%Version 1: this style won't cause trouble while compiling. it gives the name of the section and the stiff sheet
%\newpage
%\lhead[\fancyplain]{\fancyplain{}{}} \rhead[\fancyplain]{\fancyplain{}{}}
%\sectionheading{News \& Announcements}
%\newpage


%%Version 2: this will only give the stiff sheet. the section heading in the TOC has to be inserted with the command given below. Yet this will cause trouble when compiling the masterfile.
%\addtocontents{toc}{\vspace{1cm} \large\textbf{Recent Communications} \vspace{0cm} \normalsize} 

\newpage 

\thispagestyle{empty}
\vspace*{30mm}
\begin{center}
\huge HELAS  \\ News \\
\end{center}



==> caput_papers.tex <==


%%Version 1: this style won't cause trouble while compiling. it gives the name of the section and the stiff sheet
%\newpage
%\lhead[\fancyplain]{\fancyplain{}{}} \rhead[\fancyplain]{\fancyplain{}{}}
%\sectionheading{News \& Announcements}
%\newpage


%%Version 2: this will only give the stiff sheet. the section heading in the TOC has to be inserted with the command given below. Yet this will cause trouble when compiling the masterfile.
%\addtocontents{toc}{\vspace{1cm} \large\textbf{Recent Communications} \vspace{0cm} \normalsize} 


\newpage 

\pagenumbering{arabic}%
\setcounter{page}{1}%
%von mir geändert von 0 auf 1

\thispagestyle{empty}
\vspace*{30mm}
\begin{center}
\huge Scientific  \\ Papers \\
\end{center}


\newcounter{paper} 
\stepcounter{paper}
\def\code{P}
%\renewcommand\thepage {\code\arabic{paper}-\arabic{page} } 

%\newcounter{paperpage}
%\stepcoutner{paperpage}{page}
%\thepage


%\stepcounter{paper}

%\newcommand\thepapercode{\code\thepaper-\thepage}

